ChainWorld: Composing Long-Horizon Desktop Workloads from Atomic OSWorld Tasks

Computer use agents are evaluated almost exclusively on atomic desktop tasks, but realistic desktop work requires sustaining state across multiple objectives. We study this gap with ChainWorld, which composes atomic OSWorld tasks into long horizon desktop workloads through directional compatibility search while preserving the source evaluators. The resulting workload contains 347 chains of length two to four and compares two renderings of the same task sequence. In single turn evaluation, all tasks are presented together in one prompt. In multi turn evaluation, tasks are revealed one at a time. Across four current computer use agents, maximum chain completion is 31%. Multi turn evaluation improves completion for three models, but both protocols remain challenging. The two protocols also expose different failure profiles. Single turn failures concentrate on artifact precision, while multi turn failures more often reflect session management problems such as fragmented progress and later turn disengagement.

==> figures/exact_success.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{exact_success.pdf}
\vspace{-3 em}
\caption{Chain completion from isolated OSWorld tasks to ChainWorld workloads. Bars show the published OSWorld atomic task baseline together with the two ChainWorld protocols used in this paper. In single turn evaluation, all subtasks in a chain are presented together in one prompt. In multi turn evaluation, the same subtasks are revealed one at a time across turns while state carries forward. Chain completion drops sharply in both settings. The best chained result reaches 0.31, compared with an atomic task baseline of 0.79.}
\label{fig:exact_success}
\end{figure*}
 


==> figures/step_boxplots.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{step_boxplots.pdf}
\caption{Step distributions by chain length. Single turn evaluation presents the full chain in one prompt, while multi turn evaluation reveals one task per turn over the same underlying chains. The two protocols use matched per task budgets, but the step traces still reflect different turn structures, so this figure is most informative within each setting rather than as a direct behavioral comparison across settings. For multi turn chains, both the median and the spread of step counts increase with chain length, especially for Kimi 2.5. Single turn step distributions are flatter and more compressed, which suggests that many trajectories do not expand in proportion to the full stated chain.}
\label{fig:step_boxplots}
\end{figure*}


==> figures/steps_figure.tex <==
\begin{figure*}[hbt]
\centering
\includegraphics[width=\textwidth]{steps_figure.pdf}
\caption{Average steps used by chain length. The two protocols use matched per task budgets, but they differ in turn structure. In multi turn evaluation, mean step usage rises with chain length for most models. In single turn evaluation, step usage is flatter, which suggests that many trajectories do not scale their interaction budget in proportion to the full stated chain.}
\label{fig:steps}
\end{figure*}


==> math_commands.tex <==
% Common math helpers. Keep this file small and project-specific.
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\KL}{\mathrm{KL}}
\newcommand{\dataset}{\mathcal{D}}
\newcommand{\model}{\mathcal{M}}
\newcommand{\metric}{\mathcal{S}}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\params}{\theta}
\newcommand{\argmax}{\operatorname*{arg\,max}}
\newcommand{\argmin}{\operatorname*{arg\,min}}
\newcommand{\indicator}{\mathbb{I}}
\newcommand{\given}{\,\middle|\,}

